Vision Graph Prompting via Semantic Low-Rank Decomposition

Vision GNN (ViG) demonstrates superior performance by representing images as graph structures, providing a more natural way to capture irregular semantic patterns beyond traditional grid or sequence-based representations. To efficiently adapt ViG to downstream tasks, parameter-efficient fine-tuning techniques like visual prompting become increasingly essential. However, existing prompting methods are primarily designed for Transformer-based models, neglecting the rich topological relationships among nodes and edges in graph-based representations, limiting their capacity to model complex semantics. In this paper, we propose Vision Graph Prompting (VGP), a novel framework tailored for vision graph structures. Our core insight reveals that semantically connected components in the graph exhibit low-rank properties. Building on this observation, we introduce a semantic low-rank prompting method that decomposes low-rank semantic features and integrates them with prompts on vision graph topologies, capturing both global structural patterns and fine-grained semantic dependencies. Extensive experiments demonstrate our method significantly improves ViG's transfer performance on diverse downstream tasks, achieving results comparable to full fine-tuning while maintaining parameter efficiency. Our code is available at https://github.com/zhoujiahuan1991/ICML2025-VGP.

==> tables.tex <==
\begin{table}[!ht]
\centering
\caption{Performance on VTAB-1k dataset of different methods.}
\small
\vspace{3 pt}
\begin{tabular}{l|lccc}
\toprule
 & Methods & \textit{Natural} & \textit{Specialized} & \textit{Structured} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Partial}}
    & Full & - & - & - \\
    & Linear & - & - & - \\
    & Partial-1 & - & - & - \\
    & MLP-3 & - & - & - \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Extra}} 
    & Bias & - & - & - \\
    & Sidetune & - & - & - \\
    & Adapter & - & - & - \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{Prompting}}
    & VPT           & -          & -          & -          \\
    & DAM-VP        & -          & -          & -          \\
    & AutoVP        & -          & -          & -          \\
    & InsVP         & -          & -          & -          \\
    & VFPT          & -          & -          & -          \\
    & \textbf{Ours} & \textbf{-} & \textbf{-} & \textbf{-} \\
\bottomrule
\end{tabular}
\end{table}




% \begin{table*}[t] 
%     \centering
%     \caption{Ablation on effects of each component in our paradigm.}
%     \setlength{\heavyrulewidth}{1.0pt}  % 设置 \toprule 和 \bottomrule 粗细
%     \setlength{\lightrulewidth}{0.8pt}  % 设置 \midrule 粗细
%     % \setlength{\extrarowheight}{1pt} % 每行额外增加2pt高度
%     \small
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%         Node Prompt & Low Rank Node Prompt  & Global Graph Prompt & Edge Prompt & Acc. \\
%         \cmidrule(lr){1-5}
%          % \cmidrule(lr){1-1}  \cmidrule(lr){2-2}  \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
%          % \hline
% -           &-          & -          & -          & 67.2           \\
% \checkmark  &-          & -          & -          & 74.3           \\
% \checkmark  &\checkmark & -          & -          & 79.2           \\ 
% \checkmark  &\checkmark & \checkmark & -          & 83.4           \\  
% \rowcolor[gray]{0.9} 
% \checkmark  &\checkmark & \checkmark & \checkmark & \textbf{86.5}  \\  
%     \bottomrule
%     \end{tabular}
    
%     \normalsize
%     \label{table:ablation-on-main-components}
%     \vspace{0pt}
% \end{table*}

\begin{table}[!ht] 
    \centering
    \caption{Ablation on effects of each semantic low-rank prompt.}
    \setlength{\heavyrulewidth}{1.0pt}  % 设置 \toprule 和 \bottomrule 粗细
    \setlength{\lightrulewidth}{0.8pt}  % 设置 \midrule 粗细
    % \setlength{\extrarowheight}{1pt} % 每行额外增加2pt高度
    
    \small
    \vspace{3 pt}
    \begin{tabular}{c|c|c|c}
    \toprule
    $\mathbf{P_g}$  & $\mathbf{P_e}$ & $\mathbf{P_n}$ & \textit{CIFAR} \\
    % \cmidrule(lr){1-4}
     \cmidrule(lr){1-1}  \cmidrule(lr){2-2}  \cmidrule(lr){3-3}  \cmidrule(lr){4-4}
     % \hline
    -          & -          & -          & 74.3           \\
    \checkmark & -          & -          & 79.2           \\ 
    \checkmark & \checkmark & -          & 83.4           \\  
    \rowcolor[gray]{0.9} 
    \checkmark & \checkmark & \checkmark & \textbf{89.8}  \\  
    \bottomrule
    \end{tabular}
    
    \normalsize
    % \label{table:ablation-on-main-components}
    \vspace{0pt}
\end{table}



\begin{table*}[!ht]
\centering
\scriptsize % 设置整个表格为 scriptsize
\setlength{\tabcolsep}{2pt} % 调整列间距（减小列间距）
\renewcommand{\arraystretch}{1.2} % 调整行间距
\begin{tabular}{@{}c|c|ccccccc|cccc|cccccccc@{}}
\toprule
~ & ~ & \multicolumn{7}{c|}{Natural} & \multicolumn{4}{c|}{Specialized} & \multicolumn{8}{c}{Structured} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-9} \cmidrule(lr){10-13} \cmidrule(lr){14-21}
% \midrule
\rotatebox{60}{Methods} & \rotatebox{60}{Backbone} & \rotatebox{60}{CIFAR100} & \rotatebox{60}{Caltech101} & \rotatebox{60}{DTD} & \rotatebox{60}{Flowers102} & \rotatebox{60}{Pets} & \rotatebox{60}{SVHN} & \rotatebox{60}{Sun397} & \rotatebox{60}{Camelyon} & \rotatebox{60}{EuroSAT} & \rotatebox{60}{Resisc45} & \rotatebox{60}{Retinopathy} & \rotatebox{60}{Clevr-Count} & \rotatebox{60}{Clevr-Dist} & \rotatebox{60}{DMLab} & \rotatebox{60}{KITTI-Dist} & \rotatebox{60}{dSpr-Loc} & \rotatebox{60}{dSpr-Ori} & \rotatebox{60}{sNORB-Azim} & \rotatebox{60}{sNORB-Ele} \\
\midrule
Full   & ViG-M & & & & & & & & & & & & & & & & & & & \\
Linear & ViG-M & & & & & & & & & & & & & & & & & & & \\
VPT    & ViG-M & & & & & & & & & & & & & & & & & & & \\
SPT    & ViG-M & & & & & & & & & & & & & & & & & & & \\
Ours   & ViG-M & & & & & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\caption{Performance comparison across Natural, Specialized, and Structured tasks.}
% \label{tab:results}
\end{table*}

\begin{table}[!ht]
\centering
\scriptsize % 设置整个表格为 scriptsize
\setlength{\tabcolsep}{2pt} % 调整列间距（减小列间距）
\renewcommand{\arraystretch}{1.2} % 调整行间距
\begin{tabular}{c|c|ccccccc|cccc|cccccccc}
\toprule
~ & ~ & \multicolumn{7}{c|}{Natural} & \multicolumn{4}{c|}{Specialized} & \multicolumn{8}{c}{Structured} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-9} \cmidrule(lr){10-13} \cmidrule(lr){14-21}
% \midrule
\rotatebox{90}{Methods} & \rotatebox{90}{Backbone} & \rotatebox{90}{CIFAR100} & \rotatebox{90}{Caltech101} & \rotatebox{90}{DTD} & \rotatebox{90}{Flowers102} & \rotatebox{90}{Pets} & \rotatebox{90}{SVHN} & \rotatebox{90}{Sun397} & \rotatebox{90}{Camelyon} & \rotatebox{90}{EuroSAT} & \rotatebox{90}{Resisc45} & \rotatebox{90}{Retinopathy} & \rotatebox{90}{Clevr-Count} & \rotatebox{90}{Clevr-Dist} & \rotatebox{90}{DMLab} & \rotatebox{90}{KITTI-Dist} & \rotatebox{90}{dSpr-Loc} & \rotatebox{90}{dSpr-Ori} & \rotatebox{90}{sNORB-Azim} & \rotatebox{90}{sNORB-Ele} \\
\midrule
Full   & ViG-M & & & & & & & & & & & & & & & & & & & \\
Linear & ViG-M & & & & & & & & & & & & & & & & & & & \\
VPT    & ViG-M & & & & & & & & & & & & & & & & & & & \\
SPT    & ViG-M & & & & & & & & & & & & & & & & & & & \\
Ours   & ViG-M & & & & & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\caption{Performance comparison across Natural, Specialized, and Structured tasks.}
% \label{tab:results}
\end{table}


% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         ~ & Backbone & CIFAR-100 & Stanford Dogs & DTD \\ \hline
%         ViG & ViG-B-1K & 89.21 & 91.34 & 69.89 \\ \hline
%         VPT & ViG-B-1K & 74.32 & - & - \\ \hline
%         Adapter & ViG-B-1K & 82.63 & - & - \\ \hline
%         Ins-VP & ViG-B-1K & 79.65 & - & - \\ \hline
%         ViT & ViT-B-22K & 68.9 & 89.4 & 64.3 \\ \hline
%         DAM-VP & ViT-B-22K & 88.1 & 92.3 & 73.1 \\ \hline
%         GraphPrompt & ViG-B-1K & 86.49 & 92.49 & 69.20 \\ \hline
%         ~ & ~ & ~ & ~ & ~ \\ \hline
%         ~ & ~ & ~ & ~ & ~ \\ \hline
%     \end{tabular}
% \end{table*}

